Scalable Isocontour Visualization in Road Networks via Minimum-Link Paths

Isocontours in road networks represent the area that is reachable from a source within a given resource limit. We study the problem of computing accurate isocontours in realistic, large-scale networks. We propose polygons with minimum number of segments that separate reachable and unreachable components of the network. Since the resulting problem is not known to be solvable in polynomial time, we introduce several heuristics that are simple enough to be implemented in practice. A key ingredient is a new practical linear-time algorithm for minimum-link paths in simple polygons. Experiments in a challenging realistic setting show excellent performance of our algorithms in practice, answering queries in a few milliseconds on average even for long ranges.

==> tbl/tbl-range-eurocg.tex <==
% latex table generated in R 3.2.2 by xtable 1.8-0 package
% Sun Jan 10 15:39:16 2016
\begin{tabular}{lrrrr}
  \toprule
 Algorithm & Cp. & Seg. & Int. & Time \\
 \midrule
\algoExtractReachableComponent & 131 & 93\,938 & --- & 13.66 \\ 
  \algoTriangularSeparators & 219 & 1\,950 & --- & 9.50 \\ 
  \algoConnectComponents & 131 & 1\,810 & --- & 41.81 \\ 
  \algoSelfIntersections & 131 & 1\,770 & 15.27 & 40.64 \\ 
   \bottomrule
\end{tabular}

